Single-Image SVBRDF Capture with a Rendering-Aware Deep Network

Texture, highlights, and shading are some of many visual cues that allow humans to perceive material appearance in single pictures. Yet, recovering spatially-varying bi-directional reflectance distribution functions (SVBRDFs) from a single image based on such cues has challenged researchers in computer graphics for decades. We tackle lightweight appearance capture by training a deep neural network to automatically extract and make sense of these visual cues. Once trained, our network is capable of recovering per-pixel normal, diffuse albedo, specular albedo and specular roughness from a single picture of a flat surface lit by a hand-held flash. We achieve this goal by introducing several innovations on training data acquisition and network design. For training, we leverage a large dataset of artist-created, procedural SVBRDFs which we sample and render under multiple lighting directions. We further amplify the data by material mixing to cover a wide diversity of shading effects, which allows our network to work across many material classes. Motivated by the observation that distant regions of a material sample often offer complementary visual cues, we design a network that combines an encoder-decoder convolutional track for local feature extraction with a fully-connected track for global feature extraction and propagation. Many important material effects are view-dependent, and as such ambiguous when observed in a single image. We tackle this challenge by defining the loss as a differentiable SVBRDF similarity metric that compares the renderings of the predicted maps against renderings of the ground truth from several lighting and viewing directions. Combined together, these novel ingredients bring clear improvement over state of the art methods for single-shot capture of spatially varying BRDFs.

==> 3_overview.tex <==
\section{Overview}
\label{methodOverview}

\MA{Haven't touched this really, it's getting pretty out of sync possibly...}\AB{The current overview is mainly a condensed summary of the network and its losses, all illustrated in Figure~\ref{fig:overview}. We could drop this section and distribute the figures in subsequent technical sections.}\GD{I agree with removal, but we should define the capture conditions somewhere, either in the intro or as a separate section.}

Figure~\ref{fig:overview} illustrates the main components of our deep learning approach to single-image SVBRDF acquisition. 

Similarly to recent SVBRDF capture methods \cite{Aittala15,Aittala16,Riviere17}, we represent a material sample with four maps corresponding to per-pixel normal, diffuse albedo, specular albedo, and specular roughness. These maps parameterize a per-pixel Cook-Torrance BRDF model \cite{Cook82} with GGX normal distribution \cite{Walter07}, which we chose for its ability to represent a wide variety of materials (plastic, metal, wood, leather, stone, ...) \cite{Guarnera17}. In addition, this representation is compatible with many industrial renderers and middlewares, including the Allegorithmic Substance procedural texture engine \cite{Substance}, which we use to generate our training data (Section~\ref{}).
\input{figures/NetArchitectureOverview/netArchiOverview}

Our deep network follows the multi-scale \emph{U-Net} encoder-decoder architecture \cite{Ronneberger15}, which is popular for image synthesis tasks like ours \cite{rematas2017,Li17,isola17} (Figure~\ref{fig:overview}a).
We complement this network with a new \emph{secondary network} \todo{need better name} that computes global information at each scale and transmits it to the next one, as detailed in Section~\ref{}.

During training, we measure the quality of the predicted maps by comparing the resulting rendering against the rendering of the ground-truth maps, under various viewing and lighting conditions (Section~\ref{} and Figure~\ref{fig:overview}b). The motivation for this \emph{rendering loss} is to account for how the maps interact together to produce the final material appearance.
%, which is not the case with the per-map regression loss used in prior work \cite{Li17}. \AB{Not sure if we should put the finger on this particular prior work, since other existing methods used a rendering loss}

%We further improve the robustness of our approach by introducing a \emph{coherency loss}, which encourages the network to produce the same maps given two pictures of the same material under different lighting conditions (Section~\ref{} and Figure~\ref{fig:overview}c). This new loss is especially effective at diminishing highlight residuals in the maps, since the location of highlights varies with lighting.

%Our method's goal is to simplify material acquisition and to propose a way to compensate the lack of ground truth data for deep networks training in certain applications. We are in the same range of acquisition complexity as Aittala et al.~\shortcite{Aittala16} and Li et al.~\shortcite{Li17}. With one image we acquire as much information as possible about a material. We describe our choice to use the Cook-Torrance model with 4 maps to represent our data: diffuse albedo, specular albedo, roughness and normal.

%One shot material acquisition is an ill posed problem, a single picture can emphasize or mitigate some effects depending on light and view orientation. We describe our solution based on a conditional GAN composed of an encoder-decoder with skip connections generator, a conditional discriminator and secondary networks handling "global" information about the material. We also show how we personalize the loss to our problem by using renderings under multiple different lighting conditions to evaluate the difference between ground truth and output but also by enforcing a coherency constraint between similar materials.

%To train the network to this problem, we need a lot of data to alleviate all ambiguities inherent to a one-shot acquisition. We depict the use of procedural generation of materials based on parametric models defined by the "Substance" software. This method produces more than 1500 different materials represented with 4 parameter maps.

%We augment the data set by rendering these materials with randomly chosen lighting conditions, zooms and rotations. This way, we achieve approximately 50.000 rendering/ground-truth pairs for the training and testing sets. We evaluate our results against previous methods, illustrating that we are the first to treat non stochastic opaque materials and have competitive results in cases that can be treated by others. We also show the network generalization capacity through real material pictures results.


%Materials can be represented in multiple ways Ward et al.~\shortcite{Ward92}, Blinn~\shortcite{Blinn77}, Cook et al.~\shortcite{Cook82}. For our material acquisition process we need a model with multiple properties:
%\begin{itemize}
%\item The model should represent the material classes we are interested in (Plastic, Metal, Wood, Leather, ...).
%\item Collection of ground truth data of material should exist.
%\item It should be compatible with rendering software.
%\end{itemize}
%Given all these constraints we choose to use Cook-Torrance micro-facet based model with a GGX distribution \cite{Walter07}. We use 4 maps to define the BRDF parameter for each pixel. The diffuse albedo map represents the way the light is locally scattered independently of the view direction. The specular albedo map represents the reflectivity of a surface. The roughness map defines the distribution of micro facet which defines the sharpness of the specular highlight. The normal map defines local meso-scale geometry variations on the surface.
%This model can represent a wide spectrum of materials as it handles both diffuse and specular on any opaque rough spatially-varying material \cite{Guarnera17}.
%To create ground truth data using this representation we use procedural generation giving us control over the balance and size of our dataset. Finally, Cook-Torrance model is used in multiple renderers and middlewares such as Mitsuba, Optis's VRXperience or Unity or related works  \cite{Aittala15, Riviere17}.

%Inferring 4 maps of parameters out of one single image is a challenging process. As explained in \ref{methodOverview}, our method explores how deep learning helps retrieving the material model parameters and what are the influences of procedural generation on the training results. 

%Out network pipeline is to take a picture with flash as input and to output the Cook-Torrance set of maps representing the material. For the training phase, we feed the network with realistically rendered material images as input and use the ground truth maps used for the rendering as targets (see fig \ref{fig:inputData}).


==> figures/NetArchitectureOverview/netArchiOverview.tex <==
\begin{figure}[t]
\includegraphics[width=\columnwidth]{figures/NetArchitectureOverview/simplepipeline.png}
\caption{Overview of the network simplified architecture.}
\label{fig:overview}
\end{figure}

==> figures/SecondaryNetworkVisualDiff/SecondaryNetVisualDiff.tex <==
\begin{figure*}[t]

\begin{tabular}{|c|c|}
\hline 
Input & Outputs \\ 
\hline \\ 
\includegraphics[align=c, width=0.15\textwidth]{figures/SecondaryNetworkVisualDiff/0000076_PolishedMarbleFloor_01Xbrick_uneven_stones_1X1-inputs.png} &
 \begin{tabular}{cccccc}
Ground Truth & \includegraphics[align=c,width=0.15\textwidth]{figures/SecondaryNetworkVisualDiff/GT/0000076_PolishedMarbleFloor_01Xbrick_uneven_stones_1X1-targets-0-.png} & \includegraphics[align=c,width=0.15\textwidth]{figures/SecondaryNetworkVisualDiff/GT/0000076_PolishedMarbleFloor_01Xbrick_uneven_stones_1X1-targets-1-.png} & \includegraphics[align=c,width=0.15\textwidth]{figures/SecondaryNetworkVisualDiff/GT/0000076_PolishedMarbleFloor_01Xbrick_uneven_stones_1X1-targets-2-.png} & \includegraphics[align=c,width=0.15\textwidth]{figures/SecondaryNetworkVisualDiff/GT/0000076_PolishedMarbleFloor_01Xbrick_uneven_stones_1X1-targets-3-.png} &  \\ \\ 
 No Secondary &\includegraphics[align=c,width=0.15\textwidth]{figures/SecondaryNetworkVisualDiff/WithoutSecondary/0000076_PolishedMarbleFloor_01Xbrick_uneven_stones_1X1-outputs-0-.png} & \includegraphics[align=c,width=0.15\textwidth]{figures/SecondaryNetworkVisualDiff/WithoutSecondary/0000076_PolishedMarbleFloor_01Xbrick_uneven_stones_1X1-outputs-1-.png} & \includegraphics[align=c,width=0.15\textwidth]{figures/SecondaryNetworkVisualDiff/WithoutSecondary/0000076_PolishedMarbleFloor_01Xbrick_uneven_stones_1X1-outputs-2-.png} & \includegraphics[align=c,width=0.15\textwidth]{figures/SecondaryNetworkVisualDiff/WithoutSecondary/0000076_PolishedMarbleFloor_01Xbrick_uneven_stones_1X1-outputs-3-.png} &  \\ \\ 
 With Secondary &\includegraphics[align=c,width=0.15\textwidth]{figures/SecondaryNetworkVisualDiff/WithSecondary/0000076_PolishedMarbleFloor_01Xbrick_uneven_stones_1X1-outputs-0-.png} & \includegraphics[align=c,width=0.15\textwidth]{figures/SecondaryNetworkVisualDiff/WithSecondary/0000076_PolishedMarbleFloor_01Xbrick_uneven_stones_1X1-outputs-1-.png} & \includegraphics[align=c,width=0.15\textwidth]{figures/SecondaryNetworkVisualDiff/WithSecondary/0000076_PolishedMarbleFloor_01Xbrick_uneven_stones_1X1-outputs-2-.png} & \includegraphics[align=c,width=0.15\textwidth]{figures/SecondaryNetworkVisualDiff/WithSecondary/0000076_PolishedMarbleFloor_01Xbrick_uneven_stones_1X1-outputs-3-.png} &  \\ \\ 
 \end{tabular}\\
\hline
\end{tabular}


\caption{With the secondary network the specular highlight is better filled with "coherent" color pattern. Chose this material as it shows a very good example where this is very visible, there are others if needed (maybe less straight forward).}

\label{fig:SecondaryNetVisualDiff}
\end{figure*}

==> figures/SyntheticVsGT/SyntheticVsGT.tex <==
\begin{figure*}[t]

\begin{tabular}{cc}

\begin{tabular}{c}
\includegraphics[align=c, width=0.15\linewidth]{figures/SyntheticVsGT/0000039_brick_uneven_stonesXleather_tiles_0X0-inputs.png} \\
\small{Input}
\end{tabular}

 \begin{tabular}{cccccc}
\begin{sideways} \hspace{-7mm} \small{Ground truth} \end{sideways} &
\hspace{-3mm}  \includegraphics[align=c, width=0.15\linewidth]{figures/SyntheticVsGT/0000039_brick_uneven_stonesXleather_tiles_0X0-targets-0-.png} & 
\hspace{-3mm} \includegraphics[align=c, width=0.15\linewidth]{figures/SyntheticVsGT/0000039_brick_uneven_stonesXleather_tiles_0X0-targets-1-.png} & 
\hspace{-3mm} \includegraphics[align=c, width=0.15\linewidth]{figures/SyntheticVsGT/0000039_brick_uneven_stonesXleather_tiles_0X0-targets-2-.png} & 
\hspace{-3mm} \includegraphics[align=c, width=0.15\linewidth]{figures/SyntheticVsGT/0000039_brick_uneven_stonesXleather_tiles_0X0-targets-3-.png} & 
\hspace{-3mm} \includegraphics[align=c, width=0.15\linewidth]{figures/SyntheticVsGT/0000039_brick_uneven_stonesXleather_tiles_0X0-targets-rerender.png}\\ 
\vspace{-3mm}
 \\

\begin{sideways} \hspace{-8mm}  \small{Our prediction} \end{sideways} &
\hspace{-3mm} \includegraphics[align=c, width=0.15\linewidth]{figures/SyntheticVsGT/0000039_brick_uneven_stonesXleather_tiles_0X0-outputs-0-.png} & 
\hspace{-3mm} \includegraphics[align=c, width=0.15\linewidth]{figures/SyntheticVsGT/0000039_brick_uneven_stonesXleather_tiles_0X0-outputs-1-.png} & 
\hspace{-3mm} \includegraphics[align=c, width=0.15\linewidth]{figures/SyntheticVsGT/0000039_brick_uneven_stonesXleather_tiles_0X0-outputs-2-.png} & 
\hspace{-3mm} \includegraphics[align=c, width=0.15\linewidth]{figures/SyntheticVsGT/0000039_brick_uneven_stonesXleather_tiles_0X0-outputs-3-.png} & 
\hspace{-3mm} \includegraphics[align=c, width=0.15\linewidth]{figures/SyntheticVsGT/0000039_brick_uneven_stonesXleather_tiles_0X0-outputs-rerender.png} 

 \end{tabular}\\
 
 \\
 
 \begin{tabular}{c}
\includegraphics[align=c, width=0.15\linewidth]{figures/SyntheticVsGT/0000082_brick_uneven_stonesXleather_tiles_2X0-inputs.png} \\
\small{Input}
\end{tabular}

 \begin{tabular}{cccccc}
 \begin{sideways} \hspace{-8mm} \small{Ground truth} \end{sideways} &
\hspace{-3mm}   \includegraphics[align=c, width=0.15\linewidth]{figures/SyntheticVsGT/0000082_brick_uneven_stonesXleather_tiles_2X0-targets-0-.png} & 
\hspace{-3mm}  \includegraphics[align=c, width=0.15\linewidth]{figures/SyntheticVsGT/0000082_brick_uneven_stonesXleather_tiles_2X0-targets-1-.png} & 
\hspace{-3mm}  \includegraphics[align=c, width=0.15\linewidth]{figures/SyntheticVsGT/0000082_brick_uneven_stonesXleather_tiles_2X0-targets-2-.png} & 
\hspace{-3mm}  \includegraphics[align=c, width=0.15\linewidth]{figures/SyntheticVsGT/0000082_brick_uneven_stonesXleather_tiles_2X0-targets-3-.png} & 
\hspace{-3mm}  \includegraphics[align=c, width=0.15\linewidth]{figures/SyntheticVsGT/0000082_brick_uneven_stonesXleather_tiles_2X0-targets-rerender.png} \\ 
\vspace{-3mm}
 \\
 
 \begin{sideways} \hspace{-7mm}  \small{Our prediction} \end{sideways} &
\hspace{-3mm} \includegraphics[align=c, width=0.15\linewidth]{figures/SyntheticVsGT/0000082_brick_uneven_stonesXleather_tiles_2X0-outputs-0-.png} & 
\hspace{-3mm} \includegraphics[align=c, width=0.15\linewidth]{figures/SyntheticVsGT/0000082_brick_uneven_stonesXleather_tiles_2X0-outputs-1-.png} & 
\hspace{-3mm} \includegraphics[align=c, width=0.15\linewidth]{figures/SyntheticVsGT/0000082_brick_uneven_stonesXleather_tiles_2X0-outputs-2-.png} & 
\hspace{-3mm} \includegraphics[align=c, width=0.15\linewidth]{figures/SyntheticVsGT/0000082_brick_uneven_stonesXleather_tiles_2X0-outputs-3-.png} & 
\hspace{-3mm} \includegraphics[align=c, width=0.15\linewidth]{figures/SyntheticVsGT/0000082_brick_uneven_stonesXleather_tiles_2X0-outputs-rerender.png} \\

& \hspace{-3mm} \small{Normal} &\hspace{-3mm}  \small{Diffuse albedo} &\hspace{-3mm}  \small{Roughness} & \hspace{-3mm} \small{Specular albedo} &\hspace{-3mm}  \small{Re-rendering} 

 \end{tabular}

\end{tabular}


\caption{Results with synthetic data. The bricks are interesting as the results on the normals is impressive. The leather is interesting because of the spatially varying specular and roughness}

\label{fig:SubstanceDiversity}
\end{figure*}
